Schur functions and alternating sums

We discuss several well known results about Schur functions that can be proved using cancellations in alternating summations; notably we shall discuss the Pieri and Murnaghan-Nakayama rules, the Jacobi-Trudi identity and its dual (Von N{\"a}gelsbach-Kostka) identity, their proofs using the correspondence with lattice paths of Gessel and Viennot, and finally the Littlewood-Richardson rule. Our our goal is to show that the mentioned statements are closely related, and can be proved using variations of the same basic technique. We also want to emphasise the central part that is played by matrices over $\{0,1\}$ and over $\N$; we show that the Littlewood-Richardson rule as generalised by Zelevinsky has elegant formulations using either type of matrix, and that in both cases it can be obtained by two successive reductions from a large signed enumeration of such matrices, where the sign depends only on the row and column sums of the matrix.

==> topmatter.tex <==
%auto-ignore (forbid arXiv's auto-postscript generator TeXing this file alone)
% Macros that prepare for fetching and typesetting top matter for an article
% These are to be used in conjunction with marxmax.tex

\catcode`_=11 % control sequence names with this letter are private

\def\let_next{\let\next=}% this will skip one space, contrary to \letnext

\let\_authors\empty % initialise to no authors
\newtoks\this_author
\newtoks\this_addr

\newtoks\title \newtoks\MSCcodes \newtoks\CRcodes \newtoks\keywords
\newtoks\titlenote

\newtoks\DateSubmitted \newtoks\DateAccepted \newtoks\DatePublished

\newif\if_started

\def\good_break{\unskip\penalty-10\ \ignorespaces}% suggested break point


% Fetching author's information.
% Syntax: ([..] means optional)
% ( \Author[=] {<name>} 
%   [ \address[=]{<address >} ]
%   [ \email[=]{<email>} ]
%   [ \URL[=]{<WWW address>} ]
% )*
%
% result recorded in \_authors (macro)

\def\Author#1{\this_author={#1}%
  \ifx =#1\let_next\Author % allow "\Author={"
  \else \let_next\let_next \afterassignment\_author 
  \fi \next}
\def\_author
 {\this_addr=\expandafter{\default_address}%
  \ifx\next\address \let_next\get_address
  \else \ifx\next\email \let_next\get_email
  \else \ifx\next\URL \let_next\get_URL
  \else \add_author
  \fi\fi\fi \next
}

\def\address#1{\errmessage
 {\string\address\space should only follow \string\Author}}
\def\email#1{\errmessage
 {\string\email\space should only follow \string\Author}}
\def\URL#1{\errmessage
 {\string\URL\space should only follow \string\Author}}

\def\get_address{\begingroup\obeylines\get_addr}
\def\get_addr#1%
{\endgroup\this_addr={#1}%
  \ifx =#1\let_next\get_address % allow an "=" sign
  \else \let_next\let_next \afterassignment\get_ad
  \fi \next
}
\def\get_ad
{\ifx\next\email \let_next\get_email
 \else \ifx\next\URL \let_next\get_URL
 \else \add_author
 \fi\fi \next
}

\def\get_email#1%
{\ifx =#1\let_next\get_email
 \else \this_addr=\expandafter{\the\this_addr\endgraf{\tt #1}}%
   \let_next\let_next \afterassignment\after_em
 \fi \next
}
\def\after_em{\ifx\next\URL \let_next\get_URL \else \add_author \fi \next}
\def\get_URL#1%
{\ifx =#1\let_next\get_URL
 \else
  \this_addr=\expandafter{\the\this_addr\endgraf
                          {\def~{\char "7E }\tt http://#1}}%
  \let_next\add_author
 \fi \next
}

\def\add_author % Does not and should not use \next!
{\toks0=\expandafter{\_authors\\}%
 \xdef\_authors{\the\toks0 {\the\this_author
			    \noexpand\_addr{\the\this_addr}}}%
}

% Getting the article started (will be activated by \abstract or \maintext)

\def\start_art
{\vfil\eject \ifodd\pageno\else \shipout\vbox to \vsize{}\advancepageno\fi
 % force an odd page number (usually does nothing)
 \topglue 10mm plus 3 mm minus 2mm
 \centerpar{\let\\=\good_break\titlefont \baselineskip=22pt \the\title}%
 \ifx \_authors\empty \message{Warning: no authors specified.}\else
   \bigskip\centerpar
    {\subtitlefont
     \def\par{\ifhmode\endgraf\else\medskip\fi}\obeylines
     \def\_addr##1{\medskip{\addressfont\let\tt=\emailfont\let\\=\par
                   \noindent##1\endgraf}}% address information in small type
     \let\\=\bigskip% before each author
     \_authors
    }\bigskip
 \fi
 \dedication
 \aftertitlematter
 \_startedtrue
}

% Triggering the start of the article

\outer\def\abstract
{\if_started \errmessage{Abstract must be placed at start of article.}%
 \else \start_art \begingroup 
   \initabstract
	 \everypar{\everypar{}\setbox0=\lastbox}% kill first indentation
 \fi
}

\outer\def\maintext
{\if_started\medskip\endgroup\else\start_art\fi
 \afterabstractmatter
}

% Defaults

{\obeylines\gdef\default_address%
 {Universit\'e de Poitiers,  D\'epartement de Math\'ematiques,
  UFR Sciences SP2MI, T\'el\'eport~2, BP~30179, %
\ 86962 Futuroscope Chasseneuil Cedex, \ France}}

\font\titlefont=cmssbx10 scaled \magstep 3
\font\subtitlefont=cmss12
\font\addressfont=cmssi9
\font\emailfont=cmtt10

\def\initabstract
{\bigskip \ninept \sans \narrower % change of settings for entire abstract
 \leftline{\hskip\leftskip ABSTRACT}\nobreak\smallskip % formatting of heading
}

% By default MSC codes etc; follow the abstract, and dates of submission and
% such are ignored.

\def\dedication{}
\def\aftertitlematter{}

\def\afterabstractmatter
{\if &\the\MSCcodes\the\CRcodes\the\keywords\the\titlenote&\else
  {\narrower\ninept\sans
   \if &\the\MSCcodes&\else
     \hangindent=4em \noindent
     {\it Mathematics Subject Classification:\/} \the\MSCcodes.
     \par\fi
   \if &\the\CRcodes&\else
     \hangindent=4em \noindent
     {\it Computing Reviews Subject Classification:\/} \the\CRcodes.
     \par\fi
   \if &\the\keywords&\else
     \hangindent=2em \noindent{\it Keywords and Phrases:\/} \the\keywords.
     \par\fi
   \if &\the\titlenote&\else
     {\def\\{\unskip\hfil\break\ignorespaces}%
      \hangindent=2em \noindent\the\titlenote.
      \par}\fi
  }\bigskip
 \fi
}

\catcode`_=8 % Now underscores are for subscripts again

